GameArena: Evaluating LLM Reasoning through Live Computer Games

Evaluating the reasoning abilities of large language models (LLMs) is challenging. Existing benchmarks often depend on static datasets, which are vulnerable to data contamination and may get saturated over time, or on binary live human feedback that conflates reasoning with other abilities. As the most prominent dynamic benchmark, Chatbot Arena evaluates open-ended questions in real-world settings, but lacks the granularity in assessing specific reasoning capabilities. We introduce GameArena, a dynamic benchmark designed to evaluate LLM reasoning capabilities through interactive gameplay with humans. GameArena consists of three games designed to test specific reasoning capabilities (e.g., deductive and inductive reasoning), while keeping participants entertained and engaged. We analyze the gaming data retrospectively to uncover the underlying reasoning processes of LLMs and measure their fine-grained reasoning capabilities. We collect over 2000 game sessions and provide detailed assessments of various reasoning capabilities for five state-of-the-art LLMs. Our user study with 100 participants suggests that GameArena improves user engagement compared to Chatbot Arena. For the first time, GameArena enables the collection of step-by-step LLM reasoning data in the wild.

==> tables/1_intro.tex <==
\begin{table*}[t]
\centering
\caption{ Metric types define the capabilities an evaluation reflects. \textbf{Holistic} metrics apply broadly to multi-turn conversations across diverse real-world topics, while \textbf{reasoning} metrics focus on specific reasoning abilities. Interaction types describe the evaluation process. \textbf{Dynamic} evaluations involve live human interaction and preferences, while \textbf{static} evaluations are ground-truth-based or static-environment-based, which require no human involvement. }
\small
\label{tab:intro}

\begin{tabular}{c|c|c|c|}
\multicolumn{2}{c}{} & \multicolumn{2}{c}{\text{Metric Types}} \\ 
\cmidrule(lr){2-4}
& & \text{Domain-Specific} & \text{Holistic}    \\ 
\cmidrule(lr){2-4}
\multirow{2}{*}{\text{Interaction Types}}
& \text{Interactive}  &   \textbf{Game Arena}   & \text{Chatbot Arena} \\
\cmidrule(lr){2-4}
& \text{Mechanical}     &    \text{GSM8K, SmartPlay, AgentBench, PlanBench}   & \text{MT-Bench, AutoArena}  \\
\cmidrule(lr){2-4}
\end{tabular}
\end{table*}


==> tables/4_exp_akinator_deductive.tex <==
\begin{table}[htbp]
\centering
\caption{The retrospective analysis results on model's deductive reasoning capabilities reflected in Akinator game sessions. The best first appear round average and final rank average are observed in game sessions hosted by claude-3-5-sonnet-20240620, indicating strong deductive reasoning skills.}
\label{tab:4_exp_akinator_deductive}
\begin{tabular}{@{}lll@{}}
\toprule
\textbf{Model}                      & \textbf{\begin{tabular}[c]{@{}l@{}}First appear \\ round average\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Final rank \\ average\end{tabular}} \\ \midrule
\textbf{claude-3-5-sonnet-20240620} & \textbf{10.59}                                                                 & \textbf{4.75}                                                          \\
gpt-4o-2024-08-06                   & 11.12                                                                          & 5.68                                                                   \\
gemini-1.5-pro                      & 12.03                                                                          & 5.8                                                                    \\
llama-3-405b                        & 14.61                                                                          & 9.45                                                                   \\
mistral-large-latest                & 18.08                                                                          & 7.28                                                                   \\ \bottomrule
\end{tabular}
\end{table}

==> tables/4_exp_akinator_multi_hop.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}

\begin{table}[htbp]
\centering\small
\caption{The retrospective analysis results on model's multi-hop reasoning skills reflected in Bluffing game sessions. Both claude-3-5-sonnet-20240620 and gpt-4o-2024-08-06 are showing better multi-hop reasoning capabilities compared to other model evaluated. \qiyu{merge the two tables of Akinator and add separater for different reasoning capabilities}}
\label{tab:4_exp_akinator_multi_hop}
% \resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}llllll@{}}
\toprule
\textbf{Model}                      & \textbf{\begin{tabular}[c]{@{}l@{}}Disparity\\ ratio (\%)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Top 5 recall\\ rate (\%)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Top 10 recall\\ rate (\%)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Top 15 recall\\ rate (\%)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Recall\\ rate (\%)\end{tabular}} \\ \midrule
\textbf{claude-3-5-sonnet-20240620} & 0.57                                                                    & \textbf{28.54}                                                            & \textbf{31.98}                                                             & \textbf{32.90}                                                             & \textbf{32.90}                                                      \\
gpt-4o-2024-08-06                   & \textbf{0.55}                                                           & 19.87                                                                     & 22.92                                                                      & 23.52                                                                      & 23.52                                                               \\
gemini-1.5-pro                      & 0.58                                                                    & 14.47                                                                     & 15.19                                                                      & 15.19                                                                      & 15.19                                                               \\
llama-3-405b                        & 0.60                                                                    & 13.78                                                                     & 14.90                                                                      & 16.16                                                                      & 16.16                                                               \\
mistral-large-latest                & 0.62                                                                    & 4.5                                                                       & 4.88                                                                       & 4.88                                                                       & 4.88                                                                \\ \bottomrule
\end{tabular}%
% }
\end{table}

==> tables/4_exp_akinator_outcome.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{c|c|c}
\toprule
\multicolumn{3}{c}{Akinator} \\ 
\midrule
\textbf{Model} & \textbf{Avg gaming round} & \textbf{Avg win rate} \\ 
\midrule
\textbf{claude-3-5-sonnet-20240620} & 16.61 & \textbf{0.55} \\ 
gemini-1.5-pro & 16.57 & 0.51 \\ 
gpt-4o-2024-08-09 & 16.36 & 0.49 \\ 
llama-3.1-405b & 17.15 & 0.44 \\ 
mistral-large-latest & 19.99 & 0.02 \\ 
\bottomrule
\end{tabular}
\caption{Akinator game ranking
\qiyu{Consider to combine the outcome analysis results for all games to save space.}
}
\end{table}

==> tables/4_exp_akinator_retro.tex <==
\begin{table}[htbp]
\centering
\caption{The retrospective analysis of all Akinator game sessions hosted by several SOTA LLMs.}
\label{tab:4_exp_akinator_retro}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}l|llll|ll@{}}
\toprule
\textbf{Akinator}          & \multicolumn{4}{c|}{\textbf{Multi-hop reasoning}}                                                                                                                                                                                                                                                                & \multicolumn{2}{c}{\textbf{Deductive reasoning}}                                                                                                        \\ \midrule
\textbf{Model}             & \textbf{\begin{tabular}[c]{@{}l@{}}Recall\\ rate (\%)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Top 5 recall\\ rate (\%)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Top 10 recall\\ rate (\%)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Disparity\\ ratio (\%) $\downarrow$\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}First appear \\ round average\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Final rank \\ average\end{tabular}} \\ \midrule
claude-3-5-sonnet-20240620 & \textbf{27.83}                                                      & \textbf{24.58}                                                            & \textbf{27.26}                                                             & 0.57                                                                              & \textbf{11.63}                                                                 & \textbf{5.31}                                                          \\
gpt-4o-2024-08-06          & 20.32                                                               & 17.00                                                                     & 19.57                                                                      & \textbf{0.55}                                                                     & 11.96                                                                          & 6.64                                                                   \\
gemini-1.5-pro             & 19.79                                                               & 18.56                                                                     & 19.79                                                                      & 0.58                                                                              & 12.12                                                                          & 5.44                                                                   \\
llama-3-405b               & 15.90                                                               & 13.72                                                                     & 14.97                                                                      & 0.60                                                                              & 14.67                                                                          & 9.88                                                                   \\
mistral-large-latest       & 6.46                                                                & 5.90                                                                      & 6.46                                                                       & 0.62                                                                              & 18.07                                                                          & 7.11                                                                   \\ \bottomrule
\end{tabular}%
}
\end{table}

% \begin{table}[htbp]
% \centering
% \caption{The retrospective analysis of the Akinator game sessions hosted by several SOTA LLMs.}
% \label{tab:4_exp_akinator_retro}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{@{}l|llll|ll@{}}
% \toprule
% \textbf{Akinator}                                    & \multicolumn{4}{c|}{\textbf{Multi-hop reasoning}}                                                                                                                                                                                                                                                                                                                                            & \multicolumn{2}{c}{\textbf{Deductive reasoning}}                                                                                                                \\ \midrule
% \textbf{Model}                      & \textbf{\begin{tabular}[c]{@{}l@{}}Disparity\\ ratio (\%) $\downarrow$ \end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Recall\\ rate (\%)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Top 5 recall\\ rate (\%)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Top 10 recall\\ rate (\%)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}First appear \\ round average\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Final rank \\ average\end{tabular}} \\ \midrule
% claude-3-5-sonnet-20240620 & 0.57                                                                    & \textbf{32.90}                                                      & \textbf{28.54}                                                            & \textbf{31.98}                                                                                                                    & \textbf{10.59}                                                                 & \textbf{4.75}                                                          \\
% gpt-4o-2024-08-06                   & \textbf{0.55}                                                           & 23.52                                                               & 19.87                                                                     & 22.92                                                                                                                            & 11.12                                                                          & 5.68                                                                   \\
% gemini-1.5-pro                      & 0.58                                                                    & 15.19                                                               & 14.47                                                                     & 15.19                                                                                                                           & 12.03                                                                          & 5.8                                                                    \\
% llama-3-405b                        & 0.60                                                                    & 16.16                                                               & 13.78                                                                     & 14.90                                                                                                                            & 14.61                                                                          & 9.45                                                                   \\
% mistral-large-latest                & 0.62                                                                    & 4.88                                                                & 4.5                                                                       & 4.88                                                                                                                              & 18.08                                                                          & 7.28                                                                   \\ \bottomrule
% \end{tabular}%
% }
% \end{table}

% \begin{table}[htbp]
% \caption{The retrospective analysis of the Akinator game sessions hosted by several SOTA LLMs. Claude-3-5-sonnet-20240620 outperforms all other SOTA LLMs we evaluated across all the metrics in Akinator game sessions.}
% \label{tab:4_exp_akinator_retro}
% \resizebox{\columnwidth}{!}
% {
% %
% \begin{tabular}{@{}llllllll@{}}
% \toprule
% \textbf{Model}                      & \textbf{\begin{tabular}[c]{@{}l@{}}First appear \\ round average\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Final rank \\ average\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Recall\\ rate (\%)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Top 5 recall\\ rate (\%)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Top 10 recall\\ rate (\%)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Top 15 recall\\ rate (\%)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Disparity\\ ratio (\%)\end{tabular}} \downarrow \\ \midrule
% \textbf{claude-3-5-sonnet-20240620} & \textbf{10.59}                                                                 & \textbf{4.75}                                                          & \textbf{32.90}                                                      & \textbf{28.54}                                                            & \textbf{31.98}                                                             & \textbf{32.90}                                                             & 0.57                      \\
% gpt-4o-2024-08-06                   & 11.12                                                                          & 5.68                                                                   & 23.52                                                               & 19.87                                                                     & 22.92                                                                      & 23.52                                                                      & \textbf{0.55}             \\
% gemini-1.5-pro                      & 12.03                                                                          & 5.8                                                                    & 15.19                                                               & 14.47                                                                     & 15.19                                                                      & 15.19                                                                      & 0.58                      \\
% llama-3-405b                        & 14.61                                                                          & 9.45                                                                   & 16.16                                                               & 13.78                                                                     & 14.90                                                                      & 16.16                                                                      & 0.60                      \\
% mistral-large-latest                & 18.08                                                                          & 7.28                                                                   & 4.88                                                                & 4.5                                                                       & 4.88                                                                       & 4.88                                                                       & 0.62                      \\ \bottomrule
% \end{tabular}%
% }
% \end{table}


% \textbf{\#recalls} indicates the number of rounds in which the correct object appears in the object list proposed by the model. \textbf{\#top5 recalls}, \textbf{\#top10 recalls}, and \textbf{\#top15 recalls} represent the number of rounds in which the correct object appears in the proposed object list with a rank of top 5, 10, and 15, respectively.}

==> tables/4_exp_bluffing_outcome.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{c|c|c}
\toprule
\multicolumn{3}{c}{Bluffing} \\ 
\midrule
\textbf{Model} & \textbf{Avg gaming round} & \textbf{Avg win rate} \\ 
\midrule
\textbf{claude-3-5-sonnet-20240620} & 6.00 & \textbf{0.67} \\ 
gemini-1.5-pro & 5.96 & 0.60 \\ 
gpt-4o-2024-08-09 & 5.92 & 0.58 \\ 
llama-3.1-405b & 5.90 & 0.44 \\ 
mistral-large-latest & 6.00 & - \\ 
\bottomrule
\end{tabular}
\caption{Bluffing game ranking. Despite with system prompt search and optimization~\citep{khattab2024dspy}, Mistral-large~\citep{mistral2024large} fails to follow instructions and make a final prediction on the truthfulness of the users' statements within the 5-round limit.}
\end{table}


==> tables/4_exp_bluffing_retro.tex <==
\begin{table}[htbp]
\centering\small
\caption{The retrospective analysis of all Bluffing game sessions hosted by several SOTA LLMs. In many cases, Mistral-large~\citep{mistral2024large} tends to be very conservative in making predictions. Note that with a large hopping penalty and a high recall rate, LLaMA-3.1 405B tends to make bolder predictions, and its intermediate reasoning outputs tend to be slightly more inconsistent.}
\label{tab:4_exp_bluffing_retro}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}l|lll|ll@{}}
\toprule
\textbf{Bluffing}          & \multicolumn{3}{c|}{\textbf{Multi-hop reasoning}}                                                                                                                                                                                                                                                                & \multicolumn{2}{c}{\textbf{Inductive reasoning}}                                                                                                        \\ \midrule
\textbf{Model}             & \textbf{\begin{tabular}[c]{@{}l@{}}Recall\\ rate (\%)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Spearman's\\ coefficient $\downarrow$ \end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Hopping\\ penalty $\downarrow$ \end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}First appear \\ round average\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Final rank \\ average\end{tabular}} \\ \midrule
claude-3-5-sonnet-20240620 &    14.12    &     \textbf{-0.39}      &      \textbf{0.20}           &           \textbf{2.46}         &           \textbf{1.47}                                                            \\
gemini-1.5-pro             &     9.05        &          -0.22                   &                                0.23                              &                                      3.50                                           &                                1.62                                       \\
gpt-4o-2024-08-06          &                 7.64                                              &                             -0.15                                        &                                     0.44                         &                                                       3.00                          &                                             2.06                          \\
llama-3-405b               &              \textbf{19.05}                                                   &                           0.26                                          &                                0.48                              &                                                   3.00                               &                                              2.57                          \\
mistral-large-latest       &                 0.00                                               &                                 -0.20                                    &                                           0.27                   &                                   N/A                                            &                                                  1.53                    \\ \bottomrule
\end{tabular}%
}
\end{table}


==> tables/4_exp_taboo_outcome.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{c|c|c}
\toprule
\multicolumn{3}{c}{Taboo} \\ 
\midrule
\textbf{Model} & \textbf{Avg gaming round} & \textbf{Avg win rate} \\ 
\midrule
\textbf{gpt-4o-2024-08-09} & 3.19 & \textbf{0.67} \\ 
mistral-large-latest & 3.43 & 0.66 \\ 
llama-3.1-405b & 3.08 & 0.62 \\ 
claude-3-5-sonnet-20240620 & 3.36 & 0.61 \\ 
gemini-1.5-pro & 3.74 & 0.61 \\ 
\bottomrule
\end{tabular}
\caption{Taboo game ranking}
\end{table}


==> tables/4_exp_taboo_retro.tex <==
\begin{table}[htbp]
\centering\small
\caption{The retrospective analysis of all Taboo game sessions hosted by several SOTA LLMs.  
% \ax{probably should mention why llama's multi-hop is not consistent with that in akinator games session: akinatory involves some planning while in taboo it's passively answering user questions.}
}
\label{tab:4_exp_taboo_retro}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}llllll@{}}
\toprule
\textbf{Taboo}                                  & \multicolumn{3}{c}{\textbf{Multi-hop reasoning}}                                                                                                                                                                                                   & \multicolumn{2}{c}{\textbf{Abductive reasoning}}                                                                                                      \\ \midrule
\multicolumn{1}{l|}{\textbf{Model}}             & \textbf{\begin{tabular}[c]{@{}l@{}}Recall \\ rate (\%)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Top 5 recall\\ rate (\%)\end{tabular}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Top 10 recall\\ rate (\%)\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}l@{}}First appear\\ round average\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Final rank\\ average\end{tabular}} \\ \midrule
\multicolumn{1}{l|}{claude-3-5-sonnet-20240620} & 68.85                                                                & \textbf{65.82}                                                            & \multicolumn{1}{l|}{68.85}                                                                      & \textbf{1.56}                                                                 & \textbf{1.48}                                                         \\
\multicolumn{1}{l|}{gpt-4o-2024-08-06}          & 55.78                                                                & 53.68                                                                     & \multicolumn{1}{l|}{55.78}                                                                      & 2.47                                                                          & 3.83                                                                  \\
\multicolumn{1}{l|}{gemini-1.5-pro}             & 55.57                                                                & 52.58                                                                     & \multicolumn{1}{l|}{56.31}                                                                      & 2.55                                                                          & 2.44                                                                  \\
\multicolumn{1}{l|}{llama-3-405b}               & \textbf{71.22}                                                       & 65.69                                                                     & \multicolumn{1}{l|}{\textbf{70.80}}                                                             & 1.98                                                                          & 4.04                                                                  \\
mistral-large-latest                            & 66.30                                                                & 61.34                                                                     & 64.88                                                                                           & 2.05                                                                          & 4.89                                                                  \\ \bottomrule
\end{tabular}%
}
\end{table}

% \begin{table}[htbp]
% \centering\small
% \caption{The retrospective analysis of Taboo game sessions hosted by several SOTA LLMs. Claude-3-5-sonnet-20240620 outperforms all other SOTA LLMs on the \textbf{First appear round average} and \textbf{Final rank average} while llama-3-405b has leading recall rates compared to all other models.}
% \label{tab:4_exp_taboo_retro}
% \resizebox{0.9\columnwidth}{!}{%
% \begin{tabular}{@{}l|lll|ll@{}}
% \toprule
%                                     & \multicolumn{3}{c|}{\textbf{Multi-hop reasoning}}                                                                                                                                                                                                                                                                                        & \multicolumn{2}{c}{\textbf{Abductive reasoning}}                                                                                                              \\ \midrule
% \textbf{Model}                      & \textbf{\begin{tabular}[c]{@{}l@{}}Recall \\ rate (\%)\end{tabular}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Top 5 recall\\ rate (\%)\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}l@{}}Top 10 recall\\ rate (\%)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}First appear\\ round average\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Final rank\\ average\end{tabular}} \\ \midrule
% claude-3-5-sonnet-20240620 & 65.98                                                                & 63.92                                                                     & 65.98                                                                                                                              & \textbf{0.59}                                                                 & \textbf{1.41}                                                         \\
% gpt-4o-2024-08-06                   & 52.14                                                                & 50.71                                                                     & 52.14                                                                                                                     & 1.96                                                                          & 4.57                                                                  \\
% gemini-1.5-pro                      & 59.90                                                                & 58.28                                                                     & 59.90                                                                                                                  & 1.48                                                                          & 1.91                                                                  \\
% llama-3-405b                        & \textbf{75.24}                                                       & \textbf{70.87}                                                            & \textbf{75.24}                                                                                             & 1.14                                                                          & 3.24                                                                  \\
% mistral-large-latest                & 71.57                                                                & 64.59                                                                     & 68.94                                                                                               & 1.10                                                                          & 5.21                                                                  \\ \bottomrule
% \end{tabular}%
% }
% \end{table}

% \begin{table}[htbp]
% \centering
% \caption{The retrospective analysis of Taboo game sessions hosted by several SOTA LLMs. Claude-3-5-sonnet-20240620 outperforms all other SOTA LLMs on the \textbf{First appear round average} and \textbf{Final rank average} while llama-3-405b has leading recall rates compared to all other models.}
% \label{tab:4_exp_taboo_retro}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{@{}lllllll@{}}
% \toprule
% \textbf{Model}                      & \textbf{\begin{tabular}[c]{@{}l@{}}First appear\\ round average\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Final rank\\ average\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Recall \\ rate (\%)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Top 5 recall\\ rate (\%)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Top 10 recall\\ rate (\%)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Top 15 recall\\ rate (\%)\end{tabular}} \\ \midrule
% \textbf{claude-3-5-sonnet-20240620} & \textbf{0.59}                                                                 & \textbf{1.41}                                                         & 65.98                                                                & 63.92                                                                     & 65.98                                                                      & 65.98                                                                      \\
% gpt-4o-2024-08-06                   & 1.96                                                                          & 4.57                                                                  & 52.14                                                                & 50.71                                                                     & 52.14                                                                      & 52.14                                                                      \\
% gemini-1.5-pro                      & 1.48                                                                          & 1.91                                                                  & 59.90                                                                & 58.28                                                                     & 59.90                                                                      & 59.90                                                                      \\
% llama-3-405b                        & 1.14                                                                          & 3.24                                                                  & \textbf{75.24}                                                       & \textbf{70.87}                                                            & \textbf{75.24}                                                             & \textbf{75.24}                                                             \\
% mistral-large-latest                & 1.10                                                                          & 5.21                                                                  & 71.57                                                                & 64.59                                                                     & 68.94                                                                      & 71.57                                                                      \\ \bottomrule
% \end{tabular}%
% }
% \end{table}

% \begin{table}[htbp]
% \caption{The retrospective analysis of Taboo game sessions hosted by several SOTA LLMs. \textbf{First appear round average} refers to the average round number in which the model adds the correct word into the word list. \textbf{Final rank average} is the rank of the correct word in the word list proposed after the last user prompt during the game session. \textbf{Recall rate} indicates the average proportion of model proposed word lists containing the correct word during a game session.} \textbf{Top 5 recall rate}, \textbf{Top 10 recall rate}, and \textbf{Top 15 recall rate} respectively represent the average proportion of the model proposed word lists where the rank of the correct word is within the top 5, 10, and 15 positions in a game session. Claude-3-5-sonnet-20240620 outperforms all other SOTA LLMs on the \textbf{First appear round average} and \textbf{Final rank average} while llama-3-405b has leading recall rates compared to all other models.
% \label{tab:4_exp_taboo_retro}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{llllllll}
% \toprule
% \textbf{Model}                      & \textbf{\begin{tabular}[c]{@{}l@{}}First appear\\ round average\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Final rank\\ average\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Recall \\ rate (\%)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Top 5 recall\\ rate (\%)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Top 10 recall\\ rate (\%)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Top 15 recall\\ rate (\%)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Utter word \\ in list rate (\%)\end{tabular}} \\ 
% \midrule
% \textbf{claude-3-5-sonnet-20240620} & \textbf{0.59}                                                                 & \textbf{1.41}                                                         & 65.98                                                                & 63.92                                                                     & 65.98                                                                      & 65.98                                                                      & 55.89                                                                            \\
% gpt-4o-2024-08-06                   & 1.96                                                                          & 4.57                                                                  & 52.14                                                                & 50.71                                                                     & 52.14                                                                      & 52.14                                                                      & \textbf{21.43}                                                                   \\
% gemini-1.5-pro                      & 1.48                                                                          & 1.91                                                                  & 59.90                                                                & 58.28                                                                     & 59.90                                                                      & 59.90                                                                      & 45.46                                                                            \\
% llama-3-405b                        & 1.14                                                                          & 3.24                                                                  & \textbf{75.24}                                                       & \textbf{70.87}                                                            & \textbf{75.24}                                                             & \textbf{75.24}                                                             & 61.91                                                                            \\
% mistral-large-latest                & 1.10                                                                          & 5.21                                                                  & 71.57                                                                & 64.59                                                                     & 68.94                                                                      & 71.57                                                                      & 57.58                                                                            \\
% \bottomrule
% \end{tabular}%
% }
% \end{table}

==> tables/4_exp_user_rating.tex <==
\begin{table}[h]
\centering\small
\begin{tabular}{c|c}
\toprule
 Model & Avg User Rating (out of 10) \\ 
\midrule
\multicolumn{2}{c}{\textbf{Akinator}} \\ 
\midrule
gemini-1.5-pro & \textbf{6.93} \\ 
gpt-4o-2024-08-06 & 6.46 \\ 
llama-3.1-405b & 6.15 \\ 
claude-3-5-sonnet-20240620 & 6.07 \\ 
mistral-large-latest & 5.67 \\ 
\midrule
\multicolumn{2}{c}{\textbf{Taboo}} \\ 
\midrule
llama-3.1-405b & \textbf{7.32} \\ 
claude-3-5-sonnet-20240620 & 7.15 \\ 
gemini-1.5-pro & 6.56 \\ 
gpt-4o-2024-08-06 & 6.44 \\ 
mistral-large-latest & 5.00 \\ 
\midrule
\multicolumn{2}{c}{\textbf{Bluffing}} \\ 
\midrule
claude-3-5-sonnet-20240620 & \textbf{7.05} \\ 
gpt-4o-2024-08-06 & 6.78 \\ 
llama-3.1-405b & 6.75 \\ 
mistral-large-latest & 6.05 \\ 
gemini-1.5-pro & 5.77 \\ 
\bottomrule
\end{tabular}

